A Search for Predicted Astrometric Microlensing Events by Nearby Brown Dwarfs

Gravitational microlensing has the potential to provide direct gravitational masses of single, free-floating brown dwarfs, independent of evolutionary and atmospheric models. The proper motions and parallaxes of nearby brown dwarfs can be used to predict close future alignments with distant background stars that cause a microlensing event. Targeted astrometric follow up of the predicted microlensing events permits the brown dwarf's mass to be measured. Predicted microlensing events are typically found via searching for a peak threshold signal using an estimate of the lens mass. We develop a novel method that finds predicted events that instead will lead to a target lens mass precision. The main advantage of our method is that it does not require a lens mass estimate. We use this method to search for predicted astrometric microlensing events occurring between 2014 - 2032 using a catalog of 1225 low mass star and brown dwarf lenses in the Solar Neighborhood of spectral type M6 or later and a background source catalog from DECaLS Data Release 9. The background source catalog extends to $g = $ 23.95, providing a more dense catalog compared to Gaia. Our search did not reveal any upcoming microlensing events. We estimate the rate of astrometric microlensing event for brown dwarfs in the Legacy Survey and find it to be low $\sim10^{-5}$yr$^{-1}$. We recommend carrying out targeted searches for brown dwarfs in front of the Galactic Bulge and Plane to find astrometric microlensing events that will allow the masses of single, free-floating brown dwarfs to be measured.

==> meetingwithemily.tex <==
- move example and how code works into methodology (where now it feels a bit more like an afterthought)
- after saying "the purpose of..." in introduction, flow into saying that we developed a code for the purpose of checking for astrometric microlensing events)
- overlay DECaLS image over the Figure 1
- on histograms, plot "significant" data, so less white space
- dont need to say "L-Y brown dwarfs" every time. can just say "brown dwarfs" after I say L-Y first time. Complete out to 20 pc, incomplete out to 25 pcs
- contours and plot bd on top

==> thoughts.tex <==
So, the main purpose of this paper is to inform readers that we have looked through these candidate dwarfs for astrometric microlensing and did not find any events. These readers should know about astrometric microlensing and its contents (why else would they be reading this paper), but it could still be helpful to run through which equations we used. This still requires us to show where we got our information and why we used this information over other sources. However, rederiving the entirety of microlensing history isn't wise (although showing our own derivations and pointing readers to where the equations were derived is good). 


- include why not use photometric microlensing?
- in intro, when talk about sections, seems too robotic
